Attention Mechanism with Energy-Friendly Operations

Attention mechanism has become the dominant module in natural language processing models. It is computationally intensive and depends on massive power-hungry multiplications. In this paper, we rethink variants of attention mechanism from the energy consumption aspects. After reaching the conclusion that the energy costs of several energy-friendly operations are far less than their multiplication counterparts, we build a novel attention model by replacing multiplications with either selective operations or additions. Empirical results on three machine translation tasks demonstrate that the proposed model, against the vanilla one, achieves competitable accuracy while saving 99\% and 66\% energy during alignment calculation and the whole attention procedure. Code is available at: https://github.com/NLP2CT/E-Att.

==> figure_SNN_process.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95 \columnwidth]{figure_SNN_process.pdf}
    \caption{The illustration of signal process in an SNN cell.}
    \label{fig:computational_process_SNN}
\end{figure}

==> table_calls_of_operations_backup.tex <==
% % \begin{table*}[t]
% %     \centering
% %     \begin{tabular}{l||c|c|c}
% %     \hline
% %         Model & $S(x)$ & \# add & \# mul \\
% %     \hline
% %     \hline
% %     %     Dot-Product~\cite{vaswani2017attention} & $F_Q(X)F_K(X)^T$& $(l_1 + l_2)d^2+dl_1l_2$ & $(l_1 + l_2)d^2+dl_1l_2$ \\
% %     %     Dense~\cite{tay2020synthesizer} & $F_Q\sigma (F_K(X))$ & $l_1d^2+dl_1l_2$ & $l_1d^2+dl_1l_2$ \\
% %     %     Random~\cite{tay2020synthesizer} & Learnable parameters & 0 & 0 \\
% %     %     %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
% %     %   % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
% %     %     % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
% %     %     A$^3$N & $-|| F_Q(\mathbf{f}(X))-F_K(\mathbf{f}(X)) ||_1 $ & $(l_1 + l_2)\rhod+dl_1l_2$ & 0 \\
     
% %     \hline
% %     \end{tabular}
% %     \caption{Statistics on calls of additive/multiplicative operations. $d$: the model dimensionality; $\sigma$: the ReLU activation function and $\mathbf{f}$ is the binaried process; $\rho$ means the number that the index is 1, and  $\rho\ll d$ . $l$ refers to the sequence length. }
% %     \label{tab:stats_model_operation}
% % \end{table*}


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{l||c|c|c|c}
%     \hline
%         Model & \# Additive & \# Multiplicative & \ ASIC (\%) &\ FPGA (\%)\\
%     \hline
%     \hline
%         vanilla~\cite{vaswani2017attention} & $(l_1 + l_2)dk+l_1l_2k$ & $(l_1 + l_2)dk+l_1l_2k$ & 100 & 100 \\
%         Dense~\cite{tay2020synthesizer} & $l_1dk+l_1l_2k$ & $l_1dk+l_1l_2k$ & \\
%         RandInit~\cite{tay2020synthesizer} & 0 & 0 & 0 & 0 \\
%         %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
%       % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
%         % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
%         A$^3$N & $(l_1 + l_2)k\rho+l_1l_2k$ & 0 &  & \\
     
%     \hline
%     \end{tabular}
%     \caption{Statistics on calls of additive/multiplicative operations for calculating attention scores. Activations are omitted. Results are conducted when each attention module receive input $\mathbf{X} \in \mathcal{R}^{l_1 \times d}, \mathbf{Y} \in \mathcal{R}^{l_2 \times d}$. Each model gives query and key representations $\mathbf{Q} \in \mathcal{R}^{l_1 \times k}, \mathbf{K} \in \mathcal{R}^{l_2 \times k}$, and calculates alignment scores $\mathbf{A} \in \mathcal{R}^{l_1 \times l_2} $ for each head. $\rho$: ratio of values being 1 in binarized representations $\tilde{\mathbf{Q}}$ and $\tilde{\mathbf{K}}$.}
%     \label{tab:stats_model_operation}
% \end{table*}
% %2ld+l^2    2ld+l^2   ld+l^2    ld+l^2    2lq+l^2 

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{l||c|c|c}
%     \hline
%         Model & $S(x)$ & \# add & \# mul \\
%     \hline
%     \hline
%     %     Dot-Product~\cite{vaswani2017attention} & $F_Q(X)F_K(X)^T$& $(l_1 + l_2)d^2+dl_1l_2$ & $(l_1 + l_2)d^2+dl_1l_2$ \\
%     %     Dense~\cite{tay2020synthesizer} & $F_Q\sigma (F_K(X))$ & $l_1d^2+dl_1l_2$ & $l_1d^2+dl_1l_2$ \\
%     %     Random~\cite{tay2020synthesizer} & Learnable parameters & 0 & 0 \\
%     %     %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
%     %   % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
%     %     % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
%     %     A$^3$N & $-|| F_Q(\mathbf{f}(X))-F_K(\mathbf{f}(X)) ||_1 $ & $(l_1 + l_2)\rhod+dl_1l_2$ & 0 \\
     
%     \hline
%     \end{tabular}
%     \caption{Statistics on calls of additive/multiplicative operations. $d$: the model dimensionality; $\sigma$: the ReLU activation function and $\mathbf{f}$ is the binaried process; $\rho$ means the number that the index is 1, and  $\rho\ll d$ . $l$ refers to the sequence length. }
%     \label{tab:stats_model_operation}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{l||c|c}
%     \hline
%         Model & \# Additive & \# Multiplicative\\
%     \hline
%     \hline
%         vanilla~\cite{vaswani2017attention} & $(l_1 + l_2)dk+l_1l_2k$ & $(l_1 + l_2)dk+l_1l_2k$ \\
%         Dense~\cite{tay2020synthesizer} & $l_1dk+l_1l_2k$ & $l_1dk+l_1l_2k$ \\
%         RandInit~\cite{tay2020synthesizer} & 0 & 0 \\
%         %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
%       % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
%         % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
%         A$^3$N & $(l_1 + l_2)k\rho+l_1l_2k$ & 0\\
     
%     \hline
%     \end{tabular}
%     \caption{Statistics on calls of additive/multiplicative operations for calculating attention scores. Results are conducted when each attention module receive input $\mathbf{X} \in \mathcal{R}^{l_1 \times d}, \mathbf{Y} \in \mathcal{R}^{l_2 \times d}$. Each model gives query and key representations $\mathbf{Q} \in \mathcal{R}^{l_1 \times k}, \mathbf{K} \in \mathcal{R}^{l_2 \times k}$, and calculates alignment scores $\mathbf{A} \in \mathcal{R}^{l_1 \times l_2} $ for each head. $\rho$: ratio of values being 1 in binarized representations $\tilde{\mathbf{Q}}$ and $\tilde{\mathbf{K}}$.}
%     \label{tab:stats_model_operation}
% \end{table*}
%2ld+l^2    2ld+l^2   ld+l^2    ld+l^2    2lq+l^2 

% \begin{table}[t]
%     \centering
%     \begin{tabular}{l:ccr}
%     \toprule
%         \textbf{Model} & \# \textbf{add} & \# \textbf{mul} & $\Delta_A(\%)$  \\
%     % \hline
%     \midrule
%         Vanilla & $2ld^2+l^2d$ & $2ld^2+l^2d$ & 100.00~ \\
%         Dense & $ld^2+l^2d$ & $ld^2+l^2d$ & 51.10~ \\
%         RandInit & 0 & 0 & 0.00~ \\
%         %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
%       % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
%         % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
%     \cdashline{1-4}
%         E-ATT & $2ld\rho+l^2d$ & 0 & 0.44~ \\
    
%     \bottomrule
%     \end{tabular}
%     % \caption{Calls of addition (add) / multiplication (mul), and energy consumption ratio over ASIC chip \textcolor{red}{($\Delta$)} to derive attention scores in vanilla ATT~\cite{vaswani2017attention}, Dense~\cite{tay2021synthesizer}, RandInit~\cite{tay2021synthesizer}, and our model \textcolor{red}{following} \textsc{Transformer}-\textit{Base} setting.
%     \caption{Calls of addition (add) / multiplication (mul), and energy consumption ratio on ASIC chip ($\Delta_A$) of vanilla ATT~\cite{vaswani2017attention}, Dense~\cite{tay2021synthesizer}, RandInit~\cite{tay2021synthesizer}, and our model. % to derive attention scores in by referring to Table~\ref{tab:cmos}.
%     % Results are conducted over \textsc{Transformer}-\textit{Base} setting.
%     % Results are conducted when each attention module receive input $\mathbf{X} \in \mathcal{R}^{l_1 \times d}, \mathbf{Y} \in \mathcal{R}^{l_2 \times d}$. Each model gives query and key representations $\mathbf{Q} \in \mathcal{R}^{l_1 \times k}, \mathbf{K} \in \mathcal{R}^{l_2 \times k}$, and calculates alignment scores $\mathbf{A} \in \mathcal{R}^{l_1 \times l_2} $ for each head. 
%     $l$, $d$ and $\rho$ are sequential length, model size, and the ratio of nonzero values after binarization, respectively. Please refer to Appendix~\ref{appendix.energy_ratio_calculation} for more calculation details.}
%     \label{tab:stats_model_operation}
% \end{table}



\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l:ccr}
    \toprule
        \textbf{Model} & \# \textbf{add} & \# \textbf{mul} & $\Delta_A(\%)$ \\
    % \hline
    \midrule
        Vanilla & $3ld^2+2l^2d$ & $3ld^2+2l^2d$ & 100.00~ \\
        Dense & $2ld^2+2l^2d$ & $2ld^2+2l^2d$ & 67.59~ \\
        RandInit & $ld^2+l^2d$ & $ld^2+l^2d$ & 33.80~ \\
        %Factorized Dense & $H_A(F_A(X))* H_B(F_B(X))$ %& $d^2l+d(k_A+k_B)l$ & $d^2l+d(k_A+k_B)l$  \\
      % Factorized Random & $R_1R_2^T$ & $kl^2$ &  %$kl^2$\\
        % Only $l_1$ norm & $-|| (X-F_Q)-(X-F_K) ||_1$ & $2d^2l+dl^2$ & 0\\
    \cdashline{1-4}\noalign{\vskip 0.1ex}
        E-ATT & $ld^2+2ld+2l^2d$ & $ld^2 + l^2d$ & 34.10~ \\
    
    \bottomrule
    \end{tabular}
    % \caption{Calls of addition (add) / multiplication (mul), and energy consumption ratio over ASIC chip \textcolor{red}{($\Delta$)} to derive attention scores in vanilla ATT~\cite{vaswani2017attention}, Dense~\cite{tay2021synthesizer}, RandInit~\cite{tay2021synthesizer}, and our model \textcolor{red}{following} \textsc{Transformer}-\textit{Base} setting.
    \caption{Calls of addition (add) / multiplication (mul), and energy consumption ratio on ASIC chip ($\Delta_A$) of vanilla ATT~\cite{vaswani2017attention}, Dense~\cite{tay2021synthesizer}, RandInit~\cite{tay2021synthesizer}, and our model. % to derive attention scores in by referring to Table~\ref{tab:cmos}.
    % Results are conducted over \textsc{Transformer}-\textit{Base} setting.
    % Results are conducted when each attention module receive input $\mathbf{X} \in \mathcal{R}^{l_1 \times d}, \mathbf{Y} \in \mathcal{R}^{l_2 \times d}$. Each model gives query and key representations $\mathbf{Q} \in \mathcal{R}^{l_1 \times k}, \mathbf{K} \in \mathcal{R}^{l_2 \times k}$, and calculates alignment scores $\mathbf{A} \in \mathcal{R}^{l_1 \times l_2} $ for each head. 
    $l$ and $d$ are sequential length and model size, respectively. Please refer to Appendix~\ref{appendix.energy_ratio_calculation} for more calculation details.}
    \label{tab:stats_model_operation}
\end{table}

==> table_decay_factor_spiking_ratio.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l||c|c|c|c|c}
    \hline
        $\tau$ & 0.00 & 0.25 & 0.5 & 0.75 & 1.00 \\
    \hline
    \hline
        BLEU (\%) & N/A & 26.29 & \textbf{29.01} & 27.26 & N/A \\
    \hline
    \end{tabular}
    \caption{BLEU score upon IWSLT'15 En-Vi dev set with different values of decay factor $\tau$. N/A: fails to train.}
    \label{tab:decay_factor}
    
    \vspace{10pt}
    \begin{tabular}{l||c|c|c|c|c}
    \hline
        $V$ & -1.0 & -0.5 & 0.0 & 0.5 & 1.0 \\
    \hline
    \hline
        BLEU (\%) & N/A & 28.71 & \textbf{29.01} & 28.66 & N/A \\
    \hline
    \end{tabular}
    \caption{BLEU score upon IWSLT'15 En-Vi dev set with different values of spiking threshold $V$. N/A: fails to train.}
    \label{tab:spiking_threshold}
\end{table}

==> table_energy_cost.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l|c}
    \hline
        Model & Energy \\
    \hline
    \hline
        \textsc{Transformer}~\cite{vaswani2017attention} & 100\% \\
        TextCNN~\cite{kim2014Convolutional} & 25\% \\
        GRU~\cite{chung2014empirical} & 50\% \\
    \hline 
        SNN & 0.82\% \\
    \hline
    \end{tabular}
    \caption{Energy consumption of each model on sentimen analysis task. }
    \label{tab:energy_cost}
\end{table}
